Mapping Social Choice Theory to RLHF

Recent work on the limitations of using reinforcement learning from human feedback (RLHF) to incorporate human preferences into model behavior often raises social choice theory as a reference point. Social choice theory's analysis of settings such as voting mechanisms provides technical infrastructure that can inform how to aggregate human preferences amid disagreement. We analyze the problem settings of social choice and RLHF, identify key differences between them, and discuss how these differences may affect the RLHF interpretation of well-known technical results in social choice.

==> math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> scratch/workshop-extra.tex <==
\section{How much room for error does Borda count have?}\jess{for future work lol}

Here, we consider several extensions of Borda count and consider how they handle . BC + dimensions; BC + degree; BC + sampling

\subsection{Borda count}

\subsection{Borda count with axes of preference}
Suppose we collect ballots of the form ..

\subsection{Borda count with degree of preference}

\section{Experiments and Simulations}

\jess{Feels like we should probably do some lol but not sure what exactly}

\section{\jess{------ older ------}}


Let $N = \{1 \dots n\}$ be a set of individuals (or ``annotators'') providing judgments.
Let a judgment set $J \subseteq \Phi$ be a subset of a finite nonempty set $\Phi$ of propositional formulas.
Let a profile $\bm{J} = (J_1 \dots J_n)$ be a vector of judgment sets with one judgment set per annotator.

For RLHF, let $\mathcal{A}$ be a set of alternatives (e.g., potential language model outputs). We represent a preference for an output $a \in \mathcal{A}$ over output $b \in \mathcal{A}$ as the proposition $p_{a \succ b}$. For example, an annotator $i$ who provides the judgments $a \succ b$ and $b \succ c$ has the judgment set $J_i = \{p_{a \succ b}, p_{b \succ c}, p_{a \succ c} \}$.

Social choice theory discusses properties of different options for an aggregator $f: \bm{J} \mapsto 2^\Phi$, a function that maps a profile to a single judgment set.
RLHF instead learns a reward function $r: \mathcal{A} \mapsto \mathbb{R}$ that maps alternatives to a real-valued reward.
\evef{SCT learns an aggregator that maps a profile to 1 judgment set; RLHF learns a reward function that maps alternatives to rewards given a profile, not sure how to formalize best.
Here it's framed as the output being a real value, but we might want to frame it as being a single ranking.}

\subsubsection{Unanimity/Pareto Efficiency}
\begin{definition}(from handbook): 
An aggregator $f$ is unanimous if $\phi \in J_i$ for all $i \in N$ entails $\phi \in f(J)$, for all $\phi \in \Phi$ and all  $\bm{J} \in \mathcal{J}(\Phi)^n$.
    
\end{definition}

Strict application to RLHF: A reward function $r$ is unanimous if $p_{a \succ b} \in J_i$ for all $i \in N$ entails $r(a) > r(b)$, for all $(a, b) \in \mathcal{A}$ and all  $\bm{J} \in \mathcal{J}(\Phi)^n$.

However, unanimity does not seem necessary for a useful reward function due to the large space of alternatives and the fact that alternatives may be very similar. For example, if an output $a$ is always very slightly preferred to output $b$, it may be fine to prefer output $b$ if that leads to other desirable properties.

\begin{definition}
    Near-unanimity: For a pair of alternatives $a, b$, let $d_{a, b}$ be the number of alternatives $c$ such that $p_{a \succ c} \in J_i$ and $p_{c \succ b} \in J_i$. For some $k$ and $d$, a reward function is near-unanimous if $d_{a, b} < d$ for at least $k$ individuals in $N$ entails $r(a) > r(b)$, for all $(a, b) \in \mathcal{A}$ and all  $\bm{J} \in \mathcal{J}(\Phi)^n$.
\end{definition}

\subsubsection{Independence and Generalization}
\begin{definition} (From handbook)
    An aggregator $f$ is independent  if $\phi \in J_i \Leftrightarrow \phi \in J'_i$  for all $i \in N$ entails $\phi \in f(J) \Leftrightarrow \phi \in f(J')$, for all $\phi \in \Phi$ and all $J, J' \in \mathcal{J}(\Phi)^n$. (Whether $\Phi$ is accepted should only depend on the pattern of individual acceptances of $\Phi$.)
\end{definition}

\begin{definition} Strict application to RLHF:
    A reward function $r$ is independent if $p_{a \succ b} \in J_i \Leftrightarrow p_{a \succ b} \in J'_i$  for all $i \in N$ entails $p_{a \succ b} \in f(J) \Leftrightarrow p_{a \succ b} \in f(J')$, for all $(a, b) \in \mathcal{A}$ and all $J, J' \in \mathcal{J}(\Phi)^n$. (Whether $a$ is assigned higher reward than $b$ should only depend on the pattern of individual acceptances of $p_{a \succ b}$.)
\end{definition}

% Independence is not desirable because J is never complete for any single annotator, and also because we need to generalize to additional annotators

\begin{definition} (from handbook)
    A judgment set $J$ is complete if $\phi \in J$ or $\sim \phi \in J$ for all $\phi \in \Phi$.
\end{definition}

Independence is not a desirable property for RLHF because the reward model must generalize to unseen preferences. In particular, (1) judgment sets are not complete (only partial preferences are seen) and (2) the space of outputs is structured, such that we wish to infer reward for outputs never seen by the annotators.

For example, suppose one annotator gives the preference $a \succ b$, five other annotators give the preference $b \succ c$ (without giving a preference on $(a, b)$ or $(a, c)$), and five other annotators give the preference $c \succ a$ (without giving a preference on $(a, b)$ or $(b, c)$). Then $r(b) > r(c) > r(a)$ would be preferable, but the fact that $b$ is assigned higher reward than $a$ depends on $p_{b \succ c}$ and $p_{c \succ a}$, not only on $p_{a \succ b}$.

As another example, suppose there is a single annotator who provides the preference $a \succ b$. If output $c$ is very similar to $a$ and output $d$ is extremely similar to $b$, it is desirable to have a reward function that obeys $r(c) > r(d)$ despite the annotator never seeing $c$ or $d$.

More formally: Suppose individuals provide preferences on a subset $\mathcal{A}_{seen} \subset \mathcal{A}$ of all possible alternatives. Let $J_{i_{seen}}$ be annotator $i$'s expressed preferences on $\mathcal{A}_{seen}$ and $J_i$ their true (sometimes unseen) preferences on all of $\mathcal{A}$.

\begin{definition}
    A reward function $\epsilon$-generalizes if, when there is only one annotator $i$ for whom only the preferences $J_{i_{seen}}$ are seen, $p_{a \succ b} \in J_i \Leftrightarrow r(a) + \epsilon > r(b)$ for all $(a, b) \in \mathcal{A}$.
\end{definition}

% I'm pretty sure you can't have incompleteness and independence and eps-generalization.








% there are other ways we could define this distance, but I think this works for now
% if we do not assume that individuals give a well-ordered ranking (e.g. if they might give something like a > c, c > d, d > b, a > b), then the distance could also be defined as len(shortest (a,b) path).


% axioms in social choice 

% \section{Canonical Results and Impossibilities}

% social choice --- impossibility theorems 

% rlhf --- standard methods and what they implement (can probably mainly cite anand/cassidy's paper) 

% \section{Beyond Impossibilities (or something) }

% Proposition 1: ``collecting a more complex ballot is better.'' to formalize:
% \begin{itemize}
%     \item  better in what sense? --- handle multi-peaked distributions better? help differentiate between ``dinner party'' vs ``moral judgment,'' or at least handle them differently?
%     \item what is the more complex ballot? --- collecting annotations on different dimensions? 
% \end{itemize} 
% Cor of Prop 1: This is undesirable in the context of social choice (because incentivizes strategic action) 

% Proposition 2: In the context of RHLF, strategic action does not substantially worsen quality of learned pref model up to some number of people being strategic at some level, even if they coordinate


% \subsection{The Bradley-Terry MLE as Borda Count}

% Despite these foundational differences, \cite{Siththaranjan2023DistributionalPL} give an interpretation of the maximum-likelihood estimator (MLE) under the Bradley-Terry model as an implementation of Borda count, a standard voting rule from the social choice literature. 

% Standard social choice defn of Borda count is ... 

% In both cases, can be seen as implementing something like the following...
% \[
% BC(a) = \mathbb E_{\text{pop.}}\mathbb E_{b \in [A]} p(a \succ b)
% \]
% Note that this still makes the assumption of a fixed set of alternatives with $|\mathcal A| = A$.

%\evef{Missing some discussion here: why is it useful to map these problems together with redefinitions? Most basic version is that it allows us to map these problems together and thus describe how axiomatic characterization and distortion, not just generalization, are useful lenses for evaluating RLHF.}

% \paragraph{Psychological factors}
% It is well-known that human text annotations are often affected by psychological factors that are orthogonal to the content of the text itself, such as length or other structural features \jess{cites}. In that case, let 
% $r_{b, \theta}(a) = \sum_{j \in d} b_j\theta_ja_j$, where $b \in \mathbb R^d$ is a unit vector that captures cognitive biases in expressed preferences. 

% \paragraph{evaluator sampling}
% Suppose that the universe of all preferences are drawn globally from some unknown distribution. If evaluators are drawn i.i.d from this distribution, then and the bounds given by standard machine learning 

% \paragraph{Prompt sampling}

% OR: a reframing of the problem is ``given you satisfy XYZ on your samples, on what class of distributions do you also satisfy XYZ on?''


%Consistency and Condorcet-consistency are clearly distinct in the single-winner setting.\footnote{In fact, \citet{flanigan2023smoothed} show that while Borda count is \textit{consistent}, it is neither Condorcet nor smoothed-Condorcet consistent, implying a strong separation between the two axioms. Though they analyze a different noise model (Mallows), the qualitative takeaway still applies.} However, r

%Yet it is not obvious that an extension of consistency to the preference modeling setting would result in a definition that is any different from an extension of Condorcet consistency. 
